Active Learning for Non-Parametric Choice Models

We study the problem of actively learning a non-parametric choice model based on consumers' decisions. We present a negative result showing that such choice models may not be identifiable. To overcome the identifiability problem, we introduce a directed acyclic graph (DAG) representation of the choice model. This representation provably encodes all the information about the choice model which can be inferred from the available data, in the sense that it permits computing all choice probabilities. We establish that given exact choice probabilities for a collection of item sets, one can reconstruct the DAG. However, attempting to extend this methodology to estimate the DAG from noisy choice frequency data obtained during an active learning process leads to inaccuracies. To address this challenge, we present an inclusion-exclusion approach that effectively manages error propagation across DAG levels, leading to a more accurate estimate of the DAG. Utilizing this technique, our algorithm estimates the DAG representation of an underlying non-parametric choice model. The algorithm operates efficiently (in polynomial time) when the set of frequent rankings is drawn uniformly at random. It learns the distribution over the most popular items among frequent preference types by actively and repeatedly offering assortments of items and observing the chosen item. We demonstrate that our algorithm more effectively recovers a set of frequent preferences on both synthetic and publicly available datasets on consumers' preferences, compared to corresponding non-active learning estimation algorithms. These findings underscore the value of our algorithm and the broader applicability of active-learning approaches in modeling consumer behavior.

==> tex/back_up.tex <==
{{Before introducing our algorithms for active learning of the DAG representation of non-parametric choice models, it is essential to underscore certain properties of the DAG that are closely tied to choice probabilities. Specifically, we intend to explore the following two pivotal questions:
\begin{enumerate}

\item Can we completely recover the choice probabilities, i.e., the probability that item $i$ is chosen given a set $S \subseteq \universe$, from the DAG representation of non-parametric choice models?

\item Assuming we have access to the exact choice probabilities for any sets of items, what sets do we need in order to construct the exact DAG? 
\end{enumerate}
We address the first and second questions in Sections \ref{sec:choice_DAG} and \ref{sec:construct_DAG_exact}, respectively.

Regarding the first question, we demonstrate that choice probabilities can be accurately computed from the DAG. Given that choice frequencies are the sole input for constructing the DAG, this implies that the DAG representation captures the maximum amount of information that can be extracted from the input data.

Concerning the second question, we introduce a sequential process for constructing the DAG level by level, assuming access to the exact choice probabilities rather than noisy choice frequencies. While certain aspects of this construction will later be employed in learning the DAG from noisy choice frequencies in an active learning context, the process also sheds light on the challenges associated with active learning from noisy data.

Our results for the aforementioned questions show that   the DAG representation is essentially equivalent to choice probabilities, in that an exact DAG allows for the computation of choice probabilities, and vice versa. This equivalence enables straightforward consideration of optimization problems, such as assortment planning, under our DAG framework. Moreover, the DAG offers unique insights, enhancing its appeal for certain optimizations. For instance, considering that the nodes at any level \( j \) of the DAG represent the top \( j \) items for a customer segment, it becomes simpler to implement diversity constraints. These constraints could, for example, ensure the inclusion of at least the top two items from every customer segment. Additionally, the DAG can be used to enforce constraints like offering at least one of the top three choices for every customer segment.}}

\dkdeletecomment{First half is in Proposition 1 now. Second part is just one line, and might not need a lemma.}{
\begin{lemma}
\label{lem:type-set-properties}
For fixed $z$, the sets associated with the edge probability  $\edgeprob{A}{z}$, i.e.,  $\Psc_{A \oplus z} = \Set{\pi \in \Pi}{\Set{\pi(j')}{j' = 1, \ldots, j} = A, \pi(j+1) = z, p(\pi)>0}$,   are pairwise disjoint. More formally, let $A \neq A'$, and $z \notin A, z \notin A'$. Then, $\Psc_{A \oplus z} \cap \Psc_{A' \oplus z} = \emptyset$. Moreover, for any $A, z \notin A$, we have that $\sum_{A' \in \familysetnodepreR(A,z)} 
\edgeprob{A'}{z}{R}\leq \raresum$.
\end{lemma}

\begin{proof}
For the first part of the lemma, if $|A| \neq |A'|$, then $z$ is in different positions for types in $\Psc_{A \oplus z}$ and $\Psc_{A' \oplus z}$, so no type can be in both sets. Otherwise, the set of elements preceding $z$ is different in $\Psc_{A \oplus z}$ and $\Psc_{A' \oplus z}$, so again, no type can be in both sets.

Then, because the sets $\Psc_{A' \oplus z}$ for $A' \in \familysetnodepreR(A, z)$ are pairwise disjoint, we obtain that
      \[
       \sum_{A' \in \familysetnodepreR(A,z)} \edgeprob[R]{A'}{z}
      = \sum_{A' \in \familysetnodepreR(A,z)} p(\Psc^R_{A' \oplus z}) 
      \; = \;  
      p \left( \bigcup_{A' \in \familysetnodepreR(A,z)} \Psc^R_{A' \oplus z} \right)
      \; \leq \; \raresum,
      \]
      where the second step used that we are considering the total probability on a (sub-)set of rare types.
\end{proof}
}
\dkdeletecomment{saving the old approximate inclusion-exclusion lemma and proof here in case my new proof has a bug.}{
\begin{lemma}
\label{lem:sc-ie}
Let $A$ be a set of items and $z \notin A$.  Let $\mathcal{C} \subseteq \familyminus(A)$ be a set cover of $\familysetnodepreF(A,z)$, using only sets from $\familyminus(A)$, in the sense that for each $A' \in \familysetnodepreF(A,z)$, there is a set $C \in \mathcal{C}$ with $A' \subseteq C$. Then, 
\begin{equation}
\sum_{A' \in \familysetnodepreF(A,z)} \edgeprob{A'}{z}
\; \leq \; \sum_{\mathcal{B} \subseteq \mathcal{C}, \mathcal{B} \neq \emptyset} (-1)^{|\mathcal{B}| + 1} \cdot q_z(\universe \setminus \bigcap_{C \in \mathcal{B}} C)
\; \leq \; \sum_{A' \subset A} \edgeprob{A'}{z}.
\label{eq:sc-ie}
\end{equation}
\end{lemma}


\begin{proof}
For any non-empty subset $\mathcal{B} \subseteq \mathcal{C}$, we write \[
S_{\mathcal{B}} 
\; = \; \universe \setminus \bigcap_{C \in \mathcal{B}} C
\; = \; \bigcup_{C \in \mathcal{B}} (\universe \setminus C).
\]
This implies that $S_{\mathcal{B} \cup \mathcal{B}'} = S_{\mathcal{B}} \cup S_{\mathcal{B'}}$.
Because $z \notin C$ for all $C \in \mathcal{C}$ (because $\mathcal{C} \subseteq \familyminus(A)$, and $z \notin A$), we obtain that $z \in S_{\mathcal{B}}$. 
Recall that $\Theta_z (S_{\mathcal{B}})$ is the set of types choosing $z$ when offered $S_{\mathcal{B}} \ni z$. 
A type $\pi$ chooses $z$ from $\bigcup_{C \in \mathcal{B}} (\universe \setminus C)$ if and only if $\pi$ chooses $z$ from $\universe \setminus C$ for each $C \in \mathcal{B}$. 
Therefore, $\Theta_z (S_{\mathcal{B}}) = \bigcap_{C \in \mathcal{B}} \Theta_z (\universe \setminus C)$.
Applying the standard Inclusion-Exclusion formula to the sets $\Theta_z (\universe \setminus C)$, we obtain that
\begin{align*}
 p \left( \bigcup_{C \in \mathcal{C}} \Theta_z (\universe \setminus C) \right)
 & = \sum_{\mathcal{B} \subseteq \mathcal{C}, \mathcal{B} \neq \emptyset} (-1)^{|\mathcal{B}|+1} \cdot p \left( \bigcap_{C \in \mathcal{B}} \Theta_z (\universe \setminus C) \right)
\\ & = \sum_{\mathcal{B} \subseteq \mathcal{C}, \mathcal{B} \neq \emptyset} (-1)^{|\mathcal{B}|+1} \cdot p ( \Theta_z (S_{\mathcal{B}}))
\\ & = \sum_{\mathcal{B} \subseteq \mathcal{C}, \mathcal{B} \neq \emptyset} (-1)^{|\mathcal{B}|+1} \cdot q_z \left( \universe \setminus \bigcap_{C \in \mathcal{B}} C \right),
\end{align*}

where the last step used that $q_z(S) = p(\Theta_z (S))$ for all sets $S \ni z$.

We now upper- and lower-bound the left-hand side $p \left( \bigcup_{C \in \mathcal{C}} \Theta_z (\universe \setminus C) \right)$.
For the upper bound, fix an arbitrary set $C \in \mathcal{C}$, and consider a type $\pi$ in $\Theta_z (\universe \setminus C)$. Because $\pi$ ranks $z$ ahead of all of $\universe \setminus C$, there exists a set $A' \subseteq C$ such that $\pi$ ranks all of $A'$ first (in some order), then $z$, and then all items not in $A'$. {\color{blue}This is exactly the event associated with having an edge between $A'$ and $A'\cup\{z\}$. Recall that the edge probability $\edgeprob{A}{z}$ is the probability of the following set:
\[
 \Psc_{A\oplus z} :=\Set{\pi \in \Pi}{\Set{\pi(j')}{j' = 1, \ldots, j} = A, \pi(j+1) = z, p(\pi)>0}.\] 


} Because each set $C \subset A$ (because the set cover used only sets in $\familyminus(A)$) and $A' \subseteq C$, we have shown that 
$\bigcup_{C \in \mathcal{C}} \Theta_z (\universe \setminus C)
\subseteq \bigcup_{A' \subset A} \Pi_{A' \oplus z}$, and hence
\[ 
p \left( \bigcup_{C \in \mathcal{C}} \Theta_z (\universe \setminus C) \right)   
\leq \sum_{A' \subset A} \edgeprob{A'}{z}.
\] 

For the lower bound, consider a set $A' \in \familysetnodepreF(A,z)$. Because $\mathcal{C}$ is a set cover of $\familysetnodepreF(A,z)$, there exists a set $C \in \mathcal{C}, C \supseteq A'$. Any type $\pi \in \Pi_{A' \oplus z}$ ranks only $A'$ ahead of $z$. Because the assortment $\universe \setminus C$ does not contain any items of $A'$, but \emph{does} contain $z$, the type $\pi$ chooses $z$ from $\universe \setminus C$. Thus, we have shown that $\Pi_{A' \oplus z} \subseteq \Theta_z (\universe \setminus C)$. Since this holds for all $A'$, we obtain that
$\bigcup_{A' \in \familysetnodepreF(A,z)} \edgeprob{A'}{z} \subseteq \bigcup_{C \in \mathcal{C}} \Theta_z (\universe \setminus C)$,
and hence
\[ 
p \left( \bigcup_{A' \in \familysetnodepreF(A,z)} \Pi_{A' \oplus z} \right) 
\leq p \left( \bigcup_{C \in \mathcal{C}} \Theta_z (\universe \setminus C) \right).
\]

Finally, by Lemma~\ref{lem:type-set-properties}, stated below,  the sets $\Pi_{A' \oplus z}$ are pairwise disjoint, i.e., $\Pi_{A' \oplus z} \cap \Pi_{A'' \oplus z} = \emptyset$ for all $A' \neq A''$ with $z \notin A', z \notin A''$. Because of disjointness, we can write
\[ 
p \left( \bigcup_{A' \in \familysetnodepreF(A,z)} \Pi_{A' \oplus z} \right) 
= \sum_{A' \in \familysetnodepreF(A,z)} \edgeprob{A'}{z},
\]
completing the proof.
\end{proof}
}

==> tex/experiments_raw_data_NOT_PART_OF_PAPER.tex <==
\eecomment{
I just use this section to drop some graphs and data.
We can later decide what actually goes to the paper.
}

\subsection{Default Setting of the Experiments}

Unless specified otherwise, we use the following parameters
in every experiment: $n = 8$,
number of the frequent permutations
and number of rare permutations are
5 and 20 respectively. $\rho$, $\kappa$, $\delta$ and $\epsilon$
are 0.01, 0.01, 0.05, 0.001, respectively.
The errors show in the charts are average absolute error.
We do not use relative error because whenever the ground truth
is zero or close to zero (due to noise),
relative error may not well-defined.

\subsection{Error in Density Estimation}

In these experiments, we check how accurately
our algorithm estimates $q_z(S)$
for a randomly drawn $S$ of a fixed size
and a random element $z \in S$.

\subsubsection{Error as a Function of $\rho$}

In Chart~\ref{fig:density-error-n0-3-rho}, $n_0 = 3$
and in Chart~\ref{fig:density-error-n0-5-rho}, $n_0 = 5$.
In both settings, we experiment with different value for $\rho$,
from 0.005 to 0.05. Each experiment is run 1000 times
and the average absolute errors are reported in the charts.
\eecomment{In Susan's experiments, number of the runs is 100 instead of 1000,
but I think 100 runs are not enough to have a accurate enough estimation
of the average error.}
\iffalse
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{experiment-charts/fig-density-error-n0-3-rho.png}
    \caption{$n_0 = 3$.}
    \label{fig:density-error-n0-3-rho}
\end{figure}

In Chart~\ref{fig:density-error-n0-3-rho},
because truncation of the DAG dominates the error,
the impact of rho is not noticeable.
In  Chart~\ref{fig:density-error-n0-5-rho},
however, an increase in the error is observable.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{experiment-charts/fig-density-error-n0-5-rho.png}
    \caption{$n_0 = 5$.}
    \label{fig:density-error-n0-5-rho}
\end{figure}

\subsubsection{Error as a Function of $\rho$}

Similar to the previous subsection,
this subsection studies the effect of $\epsilon$
on the error.
Charts~\ref{fig:density-error-n0-3-eps}~and~\ref{fig:density-error-n0-5-eps}
show the error for $n_0 = 3$ and $n_0 = 5$, respectively.
These two charts show that the impact of $\epsilon$
is practically neglible, compared to the impact of truncation.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{experiment-charts/fig-density-error-n0-3-eps.png}
    \caption{$n_0 = 3$.}
    \label{fig:density-error-n0-3-eps}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{experiment-charts/fig-density-error-n0-5-eps.png}
    \caption{$n_0 = 5$.}
    \label{fig:density-error-n0-5-eps}
\end{figure}
\fi 




%: 0.02183444508411276, 90%: 0.026889389650324235'}




\subsubsection{Error of Truncation}

Both of the previous subsections showed that
what matters the most is $n_0$, that is,
at which level, does the algorithm truncate the DAG
(and stops building the permutations).
\eecomment{Some charts to show the data for this section are to be added.}

\subsection{Error in Estimation of Market Share}

\eecomment{TODO}
